Cryptoeconomic Security for Data Availability Committees

Layer 2 systems have received increasing attention due to their potential to scale the throughput of L1 blockchains. To avoid the cost of putting data on chain, these systems increasingly turn to off-chain data availability solutions such as data availability committees (DACs). However, placing trust on DACs conflicts with the goal of obtaining an L2 architecture whose security relies solely on the L1 chain. To eliminate such trust assumptions, we propose a DAC protocol that provides financial incentives to deter the DAC nodes from adversarial behavior such as withholding data upon request. We then analyze the interaction of rational DAC nodes and clients as a dynamic game, with a Byzantine adversary that can corrupt and bribe the participants. We also define a notion of optimality for the DAC protocols, inspired by fairness and economic feasibility. Our main result shows that our protocol is optimal and guarantees security with the highest possible probability under reasonable assumptions on the adversary.

==> analysis_risk_averse.tex <==
\subsection{Risk-Averse Nodes}
\label{sec:analysis-risk-averse}

We next prove the following theorem for risk-averse clients and nodes which have a utility function of the form $f(x) = x^\nu$, where $\nu \in (0,1)$.

\begin{theorem}
\label{thm:risk-averse-optimality}
The family of slashing functions described by Section~\ref{sec:contract} is optimal for risk-averse nodes.
\end{theorem}

%Theorems~\ref{thm:axioms} and \ref{thm:axioms-converse} are proven for risk-averse nodes in Appendix~\ref{sec:appendix-proofs-risk-averse}.
They respectively show that the slashing function of Section~\ref{sec:contract} is compliant and punishment optimal for risk-averse nodes as well.
Then, via Theorem~\ref{thm:security-two-risk-averse} below, which proves the security optimality of the slashing function for risk-averse nodes, we can conclude the proof of optimality for risk-averse nodes.
Proofs of the subsequent theorems are presented in Appendix~\ref{sec:appendix-proofs-risk-averse}.

%Theorem~\ref{thm:security-two-risk-averse} states the security optimality of the slashing function for risk-averse nodes:
%We begin by showing that the slashing function is compliant considering risk-neutral nodes.

% Proof of Lemma~\ref{lem:security-zero} for risk-averse nodes concludes the proof of Theorem~\ref{thm:axioms} for risk-averse nodes.
% We next show that the slashing function is $\epsilon$-punishment-optimal.

\begin{theorem}
\label{thm:security-two-risk-averse}
The slashing function of Section~\ref{sec:contract} is security optimal.
\end{theorem}
%Proof of Theorem~\ref{thm:security-two-risk-averse} is given in Appendix~\ref{sec:appendix-proofs-risk-averse}.

Suppose a security optimal slashing function is $(p_0,1-q^*_{p_0,\nu})$-tolerant per Definition~\ref{def:tolerant}.
Here, $q^*_{p_0,\nu}$ denotes the maximum probability across all $p_0$-adversaries such that when a query is received by a security optimal contract at some slot $t$, there are less than $k$ valid clues in the contract at slot $t+1$ with probability $q^*_{p_0,\nu}$ in the worst equilibrium.
Although Theorem~\ref{thm:security-two-risk-averse} proves the security optimality of our slashing function, unlike Theorem~\ref{thm:security-two}, it does not provide an expression for $q^*_{p_0,\nu}$.
Instead, in Theorem~\ref{thm:optimization-problem}, we identify an optimization problem whose solution is $q^*_{p_0,\nu}$.
However, for $\nu \in (0,1)$, the optimization problem is not convex.
%and there are no solvers that would yield an exact solution for all possible values of the input constants such as $p_0$, $N$, $f$ and $k$.
Thus, in lieu of solving the problem, in Theorem~\ref{thm:p0-bound}, we provide bounds on $q^*_{p_0,\nu}$ 
%on the probability given the optimal slashing function of Section~\ref{sec:contract} and risk-averse nodes.
that characterize its asymptotic behavior in terms of $\nu$ and $p_0$.

\begin{theorem}
\label{thm:optimization-problem}
For any $p_0$, $0 \leq p_0 < (N-f-k+1)(p_s-p_w)$, and $\nu \in (0,1]$, $q^*_{p_0,\nu}$ is the solution to the following optimization problem:
% Suppose a contract with an optimal slashing function receives a query at some slot $j$.
% Let $q^{\mathcal{A}}_{\mathrm{v}}$ denote the probability that given an adversary $\mathcal{A}$, there are less than $k$ valid clues in the contract at slot $j+1$ in the Nash equilibrium with the largest probability of failure. 
% Then, the largest value for $q^{\mathcal{A}}_{\mathrm{v}}$ achievable by any $p_0$-adversary $\mathcal{A}$, $0 \leq p_0 < (N-f-k+1)(p_s-p_w)$, is the solution to the following optimization problem, and hereafter denoted by $q^*_{p_0,\nu}$:

Let $\mathcal{G}$ denote the set of subsets of $[N-f]$ with $N-f-k+1$ elements.
Let $x_G$ denote variables indexed by the sets $G \in \mathcal{G}$.
\begin{equation}
\begin{aligned}
\label{eq:new-optimization-formula}
\max_{j \in [|\mathcal{G}|]} &\ \sum_{j=1}^{|\mathcal{G}|} x_G\\
\textrm{s.t.} &\ \sum_{G \in \mathcal{G}: i \in G} x_G \leq \frac{(p^i_b + p_s)^\nu-(p_s)^\nu}{(p^i_b + p_s)^\nu-(p^i_b + p_w)^\nu} \quad \forall i \in [N-f] \\
&\ \sum_{i=1}^{N-f} p^i_b \leq p_0 \\
&\ p^i_b \geq 0 \quad \forall i \in [N-f] \\
&\ x_G \in [0,1] \quad \forall G \in \mathcal{G}
\end{aligned}
\end{equation}
\end{theorem}

By Remark~\ref{remark:strong-adversary}, $q^*_{p_0,\nu}=1$ if $p_0 \geq (N-f-k+1)(p_s-p_w)$.

\begin{theorem}
\label{thm:p0-bound}
Suppose $p_0 < (N-f-k+1)(p_s-p_w)$.
Then,
\begin{IEEEeqnarray*}{rCl}
&& \frac{(p_s+p_b)^\nu-(p_s)^\nu}{(p_s+p_b)^\nu-(p_w+p_b)^\nu} \leq q^*_{p_0,\nu}, \text{ and} \\
&& q^*_{p_0,\nu} \leq 
\frac{1}{N-f-k+1}\min\left(\frac{p_0}{p_s-p_w},\frac{(p_s+p_0)^\nu-(p_s)^\nu}{(p_s+p_0)^\nu-(p_w+p_0)^\nu}\right),
\end{IEEEeqnarray*}
where $p_b = \frac{p_0}{N-f-k+1}$.
\end{theorem}

%Proof of Theorems~\ref{thm:optimization-problem} and~\ref{thm:p0-bound} are given in Appendix~\ref{sec:appendix-proofs-risk-averse}.

==> draft.tex <==

% To find the probability that the number of valid clues sent to the contract is less than $k$ in the Nash equilibrium, we first define the event $\mathcal{A}(i)$ that $\node_i$ accepts the bribe and follows the adversary's strategy.
% In this case, let $\tilde{q}_i$ denote the probability that $\node_i$ accepts the bribe, \ie, $\tilde{q}_i = \Pr[\mathcal{A}(i)]$.
% Let $Q$ denote the set of adversarial and bribed nodes, and for convenience, $Q^{-i} =  Q / \{i\}$.
% Let $R_i$ denote the number of valid clues sent to the contract by the nodes other than $\node_i$.
% Define $q_i(Q^{-i})$ as the probability that $\node_i$ takes the action $\place$ if it does not accept the bribe, and the nodes in $Q^{-i}$ are bribed.
% Given these definitions, $\node_i$'s expected payoff, $\mathcal{U}_i$ can be expressed as
% \begin{IEEEeqnarray*}{rCl}
%     \sum_{\substack{Q^{-i}:\\ [N]/[N-f] \subseteq Q^{-i} \subseteq [N]/\{i\}}} && ((1-\tilde{q}_i) \mathcal{U}^{\neg\mathcal{A}}_i(Q^{-i}) +
% \tilde{q}_i \mathcal{U}^{\mathcal{A}}_i(Q^{-i})) \\
% && \prod_{j \in [N-f]/\{i\}} (\tilde{q}_j \mathbbm{1}_{j \in Q^{-i}} + (1-\tilde{q}_j) \mathbbm{1}_{j \notin Q^{-i}})
% \end{IEEEeqnarray*}
% where,
% \begin{IEEEeqnarray*}{rCl}
%     \mathcal{U}^{\neg\mathcal{A}}_i(Q^{-i}) &=& q_i(Q^{-i}) (\sum_{j=0}^{N-1}\Pr[R_i=j|Q^{-i},\neg\mathcal{A}(i)]p^{j+1}_r-p_w) \\
%     &-& (1-q_i(Q^{-i})) (\sum_{j=0}^{N-1}\Pr[R_i=j|Q^{-i},\neg\mathcal{A}(i)] p^j_p) \\
%     \mathcal{U}^{\mathcal{A}}_i(Q^{-i}) &=& p^i_b + \sum_{\substack{b_k \in \{0,1\}\\ k \in Q^{-i}}} \\ && (q_{\left(\substack{b_k,k \in Q^{-i} \\b_i = 1}\right)} (\sum_{j=0}^{N-1} \Pr[R_i=j|Q^{-i},\mathcal{A}(i),B_k=b_k,k \in Q^{-i}]p^{j+1}_r-p_w) \\
%     &&- q_{\left(\substack{b_k,k \in Q^{-i} \\b_i = 0}\right)} (\sum_{j=0}^{N-1} \Pr[R_i=j|Q^{-i},\mathcal{A}(i),B_k=b_k,k \in Q^{-i}] p^{j}_p)),
% \end{IEEEeqnarray*}
% and,
% \begin{IEEEeqnarray*}{rCl}
%     && \Pr[R_i=j|Q^{-i},\neg\mathcal{A}(i)] \\
%     &=& \sum_{\substack{b_k \in \{0,1\}\\ k \in [N]/\{i\}}} (\mathbbm{1}_{\sum_{k \in [N]/\{i\}} b_k = j}) q_{(b_k,k \in Q^{-i})} \prod_{\substack{k \in [N]/\{i\}\\ k \notin Q^{-i}}} (b_k q_k(Q^{-k}) + (1-b_k)(1-q_k(Q^{-k}))), \\
%     && Pr[R_i=j|Q^{-i},\mathcal{A}(i),B_k=b_k,k \in Q^{-i}] \\
%     &=& \sum_{\substack{b_k \in \{0,1\}\\ k \in [N]/Q}} (\mathbbm{1}_{\sum_{k \in [N]/\{i\}} b_k = j}) \prod_{k \in [N]/Q} (b_kq_k(Q^{-k}) + (1-b_k)(1-q_k(Q^{-k})))
% \end{IEEEeqnarray*}

% Since $\node_i$ maximizes its expected payoff given other nodes' actions in the Nash equilibrium, it chooses the probabilities $\tilde{q}^*_i$ and $q^*_i(Q^{-i})$ as a function the realization of these values for all other nodes, \ie, $\tilde{q}^*_j$ and $q^*_j(Q^{-j})$ for $j \in [N-k]$, $j \neq i$, in the Nash equilibrium.
% As $\Pr[R_i=j|Q^{-i},\neg\mathcal{A}(i)]$ does not depend on $\tilde{q}_i$ or $q_i(Q^{-i})$ for any $Q^{-i} \subseteq [N]$, $\node_i$ first finds the value $q^*_i(Q^{-i})$ that maximizes $\mathcal{U}^{\neg\mathcal{A}}_i(Q^{-i})$ for each realization of $Q^{-i}$.
% Then, given the maximum value of $\mathcal{U}^{\neg\mathcal{A}}_i(Q^{-i})$ for each $Q^{-i}$, $\node_i$ can find the value $\tilde{q}^*_i$ that maximizes $\mathcal{U}_i$.
% Hence, for each node $\node_i$, there are $2^{N-f-1}$ optimizations to find $q^*_i(Q^{-i})$ for each realization of $Q^{-i}$, and there is a final expression that has to be optimized to find $\tilde{q}^*_i$.
% Solving these $(N-f)(2^{N-f-1}+1)$ equations, $\node_i$ can obtain optimal values for the probabilities $q^*_i(Q^{-i})$ and $\tilde{q}^*_i$, $i \in [N-f]$, in the Nash equilibrium.
% Finally, with these values, it can calculate the probability $q^{\mathcal{A}}_{\mathrm{v}}$ that $j+1$-security is violated in the Nash equilibrium for the given adversary $\mathcal{A}$, and, among all possible adversaries, find the one that maximizes $q^{\mathcal{A}}_{\mathrm{v}}$.

% \begin{center}
% ***
% \end{center}

% We next focus on the punishment/reward scheme of Lemma~\ref{lem:security-three}.
% Since $-p_p = \max_{m \in [N]} p^m_p < \min_{m \in [N]} p_r - p_w = p_r-p_w$, $q_i(Q^{-i}) = 1$ for all $i \in [N-f]$, $Q^{-i} \subseteq [N]$.
% In other words, all nodes that do not accept the bribe take the action $\place$.
% Moreover, the optimal adversarial strategy sets $q_{b_k,k \in Q^{-i} \\b_i = 1}=1$ for all $Q \subseteq [N]$ and takes the action $\neg\place$ for the adversarial nodes; as otherwise part of the bribe is used to incentivize the nodes to take the action $\place$.
% Finally, since the nodes are symmetric, the optimal adversarial strategy that maximizes $q^{\mathcal{A}}_{\mathrm{v}}$ distributes the total bribe $p_0$ equally to the targeted set of nodes.
% Given these observations, the only parameter to optimize is the number of nodes, $M \in [N-f]$, $M > N-f-k$, targeted by the adversary with bribes.
% (If $M \leq N-f-k$, $q^{\mathcal{A}}_{\mathrm{v}}$ becomes $0$ since in this case at least $k$ non-bribed nodes take the action $\place$.)
% Without loss of generality, suppose $\mathcal{A}$ targets the nodes $\node_1$ through $\node_M$.

% Consider $\mathcal{A}$ that offers a bribe of $p_0/M$ to $M$ nodes and requests them to take the action $\neg\place$ along with the adversarial nodes.
% Suppose each of the bribed nodes take the action $\place$ with probability $q^*$ in the Nash equilibrium, which are equal due to symmetry.
% Let $R_i$ denote the number of nodes other than $\node_i$ that take the action $\place$ in the Nash equilibrium. 
% Then, if $\node_i$ takes the action $\neg\place$, its expected payoff becomes $-p_s \Pr[R_i < k] - p_p \Pr[R_i \geq k] = -(p_s-p_p)\Pr[R_i < k] - p_p$.
% Since the nodes that do not receive bribe take the action $\place$ with probability $1$, and the nodes that are offered a bribe independently choose to reject it with probability $q^*$, it holds that
% \begin{IEEEeqnarray*}{C}
%     \Pr[R_i < k] = \sum_{j=0}^{M+f+k-N-1} {M-1 \choose j} \left(q^*\right)^j \left(1-q^*\right)^{M-1-j}.
% \end{IEEEeqnarray*}

% By definition, in the equilibrium, the probability with which each $\node_i$ chooses to reject the bribe and take the action $\place$ maximizes the formula for the expected payoff, given other node's strategy profiles:
% \begin{IEEEeqnarray*}{rCl}
%     q^* &=& \argmax_{q \in [0,1]} \left(q (-p_w+p_r) + (1-q)(-(p_s-p_p)\Pr[R_i < k] - p_p + p_b)\right) \\
%     &=& \argmax_{q \in [0,1]} (-p_p - (p_s-p_p)\Pr[R_i < k] + p_b \\
%     && + q (p_r-p_w+p_p-p_b + (p_s-p_p)\Pr[R_i < k]))
% \end{IEEEeqnarray*}
% Solving for $q^*$, we find that $p_r-p_w+p_p-p_b + (p_s-p_p)\Pr[R_i < k] = 0$, or,
% \begin{IEEEeqnarray*}{C} \sum_{j=0}^{M+f+k-N-1} {M-1 \choose j} \left(q^*\right)^j \left(1-q^*\right)^{M-1-j} = \frac{p_b}{p_s-p_p} -\frac{p_r-p_w+p_p}{p_s-p_p}
% \end{IEEEeqnarray*}
% Then, $q^{\mathcal{A}}_{\mathrm{v}}$ is given by
% \begin{IEEEeqnarray*}{C} \sum_{j=0}^{M+f+k-N-1} {M \choose j} \left(q^*\right)^j \left(1-q^*\right)^{M-j}.
% \end{IEEEeqnarray*}
% The expression for $q^{\mathcal{A}}_{\mathrm{v}}$ is maximized for $M = N-f-k+1$, which gives the maximum possible value for $q^{\mathcal{A}}_{\mathrm{v}}$ over all possible adversaries:
% \begin{IEEEeqnarray*}{C} \left(\frac{p_0}{(N-f-k+1)(p_s-p_p)} -\frac{p_r-p_w+p_p}{p_s-p_p}\right)^{\frac{N-f-k+1}{N-f-k}}
% \end{IEEEeqnarray*}

%\begin{lemma}
% \label{lem:security-five}
% Consider the reward/punishment scheme of Lemma~\ref{lem:security-three}, and the subgame where a query is received by the contract at slot $j$.
% Suppose there are $N$ nodes, $k \leq N-f$, and $p_0$ is such that
% \begin{equation*}
% (N-f-k+1)(p_r-p_w+p_p) < p_0 < (N-f-k+1)(p_s-p_w-p_r)
% \end{equation*}
% Then, for all $p_0$-adversaries $\mathcal{A}$, the probability $q^{\mathcal{A}}_{\mathrm{v}}$ that $j+1$-security is violated in any Nash equilibria is upper bounded by \begin{IEEEeqnarray*}{C}
%     q^{\mathcal{A}}_{\mathrm{v}} \leq \frac{p_0}{(N-f-k+1)(p_s-p_p)} - \frac{p_r-p_w+p_p}{p_s-p_p}.
% \end{IEEEeqnarray*}
% \end{lemma}

% \begin{proof}
% Consider an adversary $\mathcal{A}$ that offers a bribe of $p^i_b$ to some node $\node_i$.
% Suppose $j+1$-security is violated with probability at most $q^{\mathcal{A}}_{\mathrm{v}}$ in any Nash equilibria.
% If $\node_i$ takes the action $\place$, its payoff becomes $p_r-p_w$.
% On the other hand, if it takes the action $\neg\place$, its expected payoff becomes $-p_p (1-q^{\mathcal{A}}_{\mathrm{v}}) - p_s q^{\mathcal{A}}_{\mathrm{v}}$.
% Then, $\node_i$ takes the action $\neg\place$ with positive probability in any Nash equilibria only if $(p_r-p_w) \leq p^i_b-p_p (1-q^{\mathcal{A}}_{\mathrm{v}}) - p_s q^{\mathcal{A}}_{\mathrm{v}}$, \ie, $p^i_b \geq (p_r-p_w+p_p) + (p_s-p_p) q^{\mathcal{A}}_{\mathrm{v}}$.

% For $j+1$-security to be violated with positive probability, at least $N-f-k+1$ nodes must choose the action $\neg\place$ with positive probability as part of their strategies in the Nash equilibrium.
% However, in this case, each of these $N-f-k+1$ nodes should have been offered a bribe of at least $(p_r-p_w+p_p) + (p_s-p_p) q^{\mathcal{A}}_{\mathrm{v}}$.
% Since the total bribe that can be offered is $p_0$, it must hold that $(N-f-k+1) ((p_r-p_w+p_p) + (p_s-p_p) q^{\mathcal{A}}_{\mathrm{v}}) \leq p_0$.
% Rearranging the terms, we obtain the upper bound given by Theorem statement on the probability $q^{\mathcal{A}}_{\mathrm{v}})$.
% \end{proof}

% \begin{lemma}
% \label{lem:security-three}
% Consider the following reward/punishment scheme: 
% \begin{IEEEeqnarray*}{rCl}
% p^m_p &=& p_p \text{ if } m \geq k \\
% p^m_p &=& p_s \text{ if } m < k \\ 
% p^m_r &=& p_r \ \forall m \in [N] \\
% 0 &<& p_r-p_w+p_p
% \end{IEEEeqnarray*}
% Consider a $(p_0,p_1)$-adversary such that
% \begin{equation*}
% p_1 < \min{(p_f,p_{\mathrm{comp}})-p_c}, \quad\quad p_0 < (N-f-k+1)(p_r-p_w+p_p).
% \end{equation*}
% Suppose there are $N$ nodes, and $k \leq N-f$. 
% Then, $4$-security is satisfied in any Nash equilibria.

% In addition to the assumptions above, if
% \begin{equation*}
% p_1<p_c,\quad\quad p_0<(N-f-k+1)(p_w-p_r),
% \end{equation*}
% then, $4$-security is satisfied without the use of the contract in any Nash equilibria.
% \end{lemma}

% Lemma~\ref{lem:security-three} shows that the two-stage punishment scheme is sufficient to ensure security with probability $1$ if the total amount of bribe is small.
% Following lemmas show that it can also guarantee a positive probability unless $p_0$ is large enough to cover the slashing costs for $\Theta(N)$ nodes.

% The reward/punishment scheme proposed by Corollary~\ref{cor:security-two} ensures that for any adversary with a limited budget, there exists a sufficiently large DAC that can provide security in all equilibria.
% However, this scheme could slash a node's collateral even when security is satisfied as it treats each node independently.
% An ideal contract should tolerate nodes that are temporarily offline, and keep the punishment small unless security is violated.
% In this context, we propose a two stage punishment scheme: $p^m_p = p_p$ if $m \geq k$, \ie, there are sufficiently many valid clues sent to the contract, and $p^m_p = p_s$, if $m < k$.

% \begin{proof}[Proof of Theorem~\ref{thm:security-one}]
% We first consider the case $p_1 < \min{(p_f,p_{\mathrm{comp}})-p_c}$ and $p_0 < (N-f-k+1)(p_r - p_w + p_s)$.
% If a query is received by the contract at slot $j$, and $\node$ takes the action $\place$ at slot $j+1$, the game is terminated and each of the res payoff becomes $p_r-p_w$.
% Otherwise, if $\node$ takes the action $\neg\place$, then the game is again terminated, and $\node$'s payoff becomes $-p_s$.
% As $p_r-p_w>-p_s$, if $\node$ is offered a bribe less than $p_r-p_w+p_s$, it chooses the action $\place$ at slot $i+1$ in any subgame where a query is received by the contract at slot $i \in \mathbb{N}$.
% Since $p_s+p_r-p_w \geq p_0$, $\node$ chooses the action $\place$ at slot $i+1$ in any subgame where a query is received by the contract at slot $i \in \mathbb{N}$.

% Suppose $\client$ is not corrupted, and $\node$ does not send a valid clue to $\client$ over the network by slot $3$.
% Then, if $\client$ does not take the action $\query$ by slot $2$, $\client$'s payoff becomes at most $p_1$.
% Conversely, if $\client$ takes the action $\query$ by slot $2$, it obtains a payoff of at least $\min(p_f,p_\mathrm{comp})-p_c$ when the game is terminated.
% Hence, if $\node$'s strategy profile is to avoid sending a valid clue to $\client$ over the network by slot $3$, since $\min(p_f,p_\mathrm{comp})-p_c>p_1$, $\client$ chooses to take the action $\query$ by slot $2$, and its payoff becomes at least $\min(p_f,p_\mathrm{comp})-p_c$.
% In this case, the query is received by the contract by slot $2$.

% Finally, if $\node$ sends a valid clue to $\client$ over the network by slot $3$, $4$-security is satisfied.
% Conversely, if $\node$ does not send a valid clue to $\client$ over the network by slot $3$, $\client$ chooses the action $\query$ by slot $2$, in which case $\node$ chooses the action $\place$ by slot $3$.
% Consequently, $4$-security is satisfied in any Nash equilibria of the game.

% We next consider the case $p_1<p_c$ and $p_0<p_w-p_r$ are satisfied besides the earlier two conditions.
% As the observations made above hold in this case as well, in the subgame where $\client$ takes the action $\query$ at any slot $i$, $\node$'s payoff becomes at least $p_r-p_w$ if it takes the action $\place$ at slot $i+1$, and at most $p_0-p_s$ otherwise.
% As $p_0<p_s-p_w+p_r$, $\node$ always takes the action $\place$ at slot $i+1$.

% If $\node$ chooses to send a valid clue to $\client$ by slot $3$ as part of its strategy, and $\client$ takes the action $\query$ at any slot $i \in \mathbb{N}$, its payoff becomes at most $p_f-p_c+p_1$ as $\node$ always takes the action $\place$ at slot $i+1$ in this case.
% Conversely, if $\client$ does not take the action $\query$ before terminating the game, its payoff becomes $p_f$.
% Since $p_1<p_c$, if $\node$ chooses to send a valid clue to $\client$ by slot $3$, $\client$ does not send the query to the contract before terminating the game, and obtains a payoff of $p_f$.
% In this case, $\node$'s payoff becomes $0$.

% Finally, if $\node$ chooses to not send a valid clue to $\client$ over the network by slot $3$, $\client$ takes the action $\query$ by slot $2$, in which case $\node$'s payoff becomes at most $p_0+p_r-p_w$.
% As $p_0 + p_r - p_w < 0$, in any Nash equilibria, $\node$ chooses to send a valid clue to $\client$ over the network by slot $3$, and $\client$ does not take the action $\query$ at any slot.
% Hence, under the two additional assumptions, $4$-security is satisfied without the use of the contract in any Nash equilibria.
% \end{proof}

==> meeting_notes.tex <==
\section{Meeting 5/26}
\begin{itemize}
    \item Proof of wrong vector element for KZG (we want a hiding proof) - equivalent to proof of non-inclusion for accumulators.
    \item Impossibility result for the minimum data required for updating the witness extends to accumulators (or VCs) with only additions, but proofs of non-inclusion.
    \item Graph the minimum probability for data recovery given adversarial bribe and the punishment/reward parameters.
    \item Can our slashing mechanism through the on-chain contract dis-incentivize centralization of storage (which can lead to data retrievability attacks)?
    \item Bribe quantification: Honest node receives a bribe, finds the optimal action given other node's bribes and optimal actions (Nash equilibrium), and selects the bribe distribution that minimizes the probability of data recovery. 
    (Due to symmetry, adversary only has to determine how many nodes to bribe, a single parameter of freedom, since the bribes will have to be equal.)
    In this case, there is no information asymmetry: Given that the bribe amount is known, there is an optimal way to allocate the bribe known by every node.
    (Model needs to be updated appropriately.)
    \item For the adversarial nodes, the same strategy as the one above can be used. Honest nodes find the optimal action given the other node's bribes, their optimal actions and the adversarial strategy (Nash equilibrium), then the adversary chooses the best strategy for the bribes and the adversarial nodes (which can be a randomized strategy). 
    \item Expand the use-case discussion to incorporate the SNARK proof as discussed. Clients assume the burden of placing a query with the hash of their accounts. Here, the hash provides anonymity for their accounts, and the fact that the account hashes are placed by the client ensures that the data cost of the nodes is not high, and is indeed limited to the proof size.
    \item The lack of information asymmetry is not specific to the case where adversary's allocation is one-shot since honest nodes can simulate the future actions like the adversary (More thinking is needed.) 
    However, information asymmetry would be a problem if the adversary, e.g., its nodes, can change behavior after the honest nodes take action.
    \item Reducing the multi-stage game to a multi-party prisoner's dilemma (?)
    \item Highlight the means of the bribe (?).
\end{itemize}

\section{Meeting 6/2}
\begin{itemize}
    \item Research Arweave's incentive mechanism to avoid storage delegation. Check if their parameters fit into our model, or if we can inform their parameters with our model.
    \item Write the two lemmas for the optimal adversarial action behind Lemma 2: Symmetry and setting $q_{\mathrm{reply}}$ to zero. 
    \item Check out Tim Roughgarden's paper, update the model section, include the axioms that guide our design choices.
    \item For now, we keep the static adversary model where the adversary loses the bribe after offer.
    \item Extension of the single-shot game to multiple games, adversary can re-use the unused bribes offered at each game. Do we allow adversarial strategies that can coordinate across multiple games? This might not matter since the optimal strategy is to request nodes to withhold data from the contract.
    \item Simplify the formulas with the parameter values selected to satisfy the axioms.
    \item Graph the bribe required as the number of nodes increase for a given level of security and given that the other parameters are fixed by the axioms.
    \item Adaptive adversary discussion can be added later, or as part of a different project. It is unclear if the new bribery model qualifies as adaptive, it can potentially replace the existing static adversary model description. 
\end{itemize}

\section{Meeting 6/11}

\begin{itemize}
    \item Arweave
    \item Major changes in the analysis section
    \item Axioms - priority order of axioms
    \item Repeated games and the issue of deviation by the adversary and the nodes - Adversary can coordinate across different game instances - Probability decays polynomially in latency :(
    \item Calculations
\end{itemize}

\textbf{Action Items}
\begin{itemize}
    \item The security axiom should be expressed as an evaluation parameter for the contract and the reward/punishment function. 
    \item Prove that our contract achieves the best possible security, \ie, minimum error probability, given any adversary that satisfies the rudimentary axioms.
    \item Without repeated games, adversary cannot support the equilibrium as one party always has the incentive to deviate. 
    In this case, repeated games with a tit-for-tat strategy are necessary to ensure that the equilibrium can be supported. 
    \item Talk about the multi-shot version of the game, and how the gain in security is small: Error probability scales as $O(1/l)$ as latency $l$ grows.
    Same argument for the repeated games also applies to the multi-shot game.
    \item Repeated games make sense if the adversary and the nodes can stake multiple times back to back, even after they lose their collateral due to a security violation. 
    Some discussion is needed to emphasize this point.
    \item We can perhaps achieve smaller error probabilities for risk-averse nodes. Do the same calculations apply to risk-averse nodes? Is our contract still optimal?
    \item Read and present the Permacoin paper in the crypto-reading group.
    \item Discussion for the next meeting: Can we somehow capture the property of not having to use the contract as an axiom? For instance, contract should ensure that it is not used in an equilibria without a strong adversary offering high bribes.
    \item For the future: Aptos designers are worried about having to access too many data points to update the data structure for the key-value map, \eg, their vector commitment.
    State reads and writes are costly, and a better design that minimizes the access to the state after updates is needed.
\end{itemize}

\section{Meeting 6/23}
\begin{itemize}
    \item Revised model, protocol and analysis.
    \item New notions of optimality.
    \item Proving new notions of optimality.
    \item Upper bound on the probability of security failure shown on the protocol, lower bound shown on any protocol.
    \item Difficulties with risk-averse adversaries.
    \item Next step: Complete the risk-averse architecture.
    \item Next step: Repeated game
\end{itemize}

\section{Meeting 6/30}
\begin{itemize}
    \item Added remark for the multi-shot games, a new section on repeated games.
    \item Optimal adversary for risk-averse nodes (not convex), shall we leave it at the optimization problem? We can still prove that the contract is optimal, but might not find out the exact value.
    We can treat it as a known solution $q^*$ of the optimization problem, and use this value as such.
    \item Upper bound: trivial one is not helpful, full characterization still requires solving an optimization problem (at least, this is convex).
    \item Risk-averse nodes do not provide much extra security, even given the best contract.
    \item Proof-read the analysis section.
    \item SBC response, alphabetic task distribution?
    \item Check out papers on risk-aversion coefficient.
    \item Evaluation graph: To show overpay is not too much.
    \item Cite the original paper.
\end{itemize}

\section{Meeting 7/29}
\begin{itemize}
    \item Feedback on the paper
    \item Shall we have more references?
    \item Title: the word 'accountability' does not show up in the main text so removed from the title.
    \item Negligible probability problem, how much change should be made to the text? - Can we state that non-negligible probabilities include a plus negl term? - Theorem statement.
    \item Authors, submission.
    \item Graph and the table, what shall we plot? What about bribes for different $\nu$ as the number of DAC nodes change?
    \item Main changes: expanded game section, merging of risk-neutral and risk-averse sections, moving of the approximation to appendix.
\end{itemize}   

TODO Items for Monday: 
\begin{itemize}
    \item Add discussion on off chain data with data availability sampling. - Done
    \item Cite the two blog posts on Celestium and the ransom attack in the indicated place. This is important, compare our scheme with the guarantees of DAS, is DAS really trust-minimized?? - Done
    \item Change the graph, fix the code for the graph. We are now plotting only the lower bounds for $\nu=0.1, 0.5, 0.8, 1$ with different colors. Gap between the lower and upper bounds becomes large for small $\nu$. Update the graph caption accordingly, update the table in the evaluation accordingly with both upper and lower bounds!
    \item Talk about how the bribe is high for security to degrade to 99.9 percent, the fact that adversary has to pay this high bribe consistently to violate security for multiple client queries. - Done
    \item Don't forget to change the concrete failure probability to $\epsilon = 0.001$ in the Appendix (especially the Appendix referred by the Evaluation section) Evaluation and Introduction! - Done
    \item In the introduction and evaluation, don't forget to add the price of Ethereum in terms of USD. We might want to write all prices in both ETH and USD, for instance, the collateral $p_s$ in both ETH and USD within introduction and evaluation sections. - Done
    \item For the negligible probability problem, we should either state that we assume Ethereum is secure, or talk about grouping the negl term with the non-negl probabilities. We should state what this probability states, \ie, the fact that cryptographic primitives underlying the contract might break, causing errors in the contract. 
    We should not explicitly write negl terms everywhere to avoid cluttering the descriptions. - Done
    \item In the analysis of the optimal contract section, explicitly state that Theorem 5 is for risk-neutral nodes in the theorem body. Then, in the final paragraph, explicitly write out the term for the failure probability of risk-neutral nodes before discussing the fact that this probability is hard to write out in closed form for risk-averse nodes.
    Go over this section again briefly to observe if the main points are well-described, especially the fact that theorems apply to both risk-neutral and risk-averse nodes. - Done
    \item In the ePrint submission, we might still want to keep theorem statements in a separate section for ease of reading.
    \item Don't forget to upload the code.
    \item One needs to state what $\nu$ represents, \ie, the risk-aversity of nodes, whenever it is mentioned, especially at the beginning of a paragraph. - Done
    \item Ideally, paragraphs should start with a sentence that explains what the paragraph will explain. This is especially important for remarks and remark-like paragraphs of the analysis. Go over them and add explanatory sentences at appropriate places. - Done
    \item Fix evaluation, remove the graph. - Done
\end{itemize}

==> scratchpad_analysis.tex <==
% We next generalize the DAC protocol to multiple DAC members.
% Suppose there are $N$ DAC members, and the contract slashes the funds of a DAC member if it fails to respond to a complaint in time.
% Then, the following lemma holds:

% \begin{lemma}
% \label{lem:security-multiple}
% Suppose
% \begin{equation*}
% \Tconf+\Texp+\Delta < \Tcutoff < \Tda,
% \end{equation*}
% \begin{equation*}
% p_1 < \min{(p_f,p_{\mathrm{comp}})-p_c},
% \end{equation*}
% \begin{equation*}
% p_0 < N(p_s - p_w).
% \end{equation*}
% Suppose the DAC consists of $N$ members and there is a single client. 
% Then, the DAC security of Definition~\ref{def:dac-security} is satisfied in all Nash equilibria.

% In addition to the assumptions above, if,
% \begin{equation*}
% p_1<p_f-\max{(p_f,p_{\mathrm{comp}})}+p_c,
% \end{equation*}
% and,
% \begin{equation*}
% p_0 < N\min{(p_s,p_w)},
% \end{equation*}
% then the normal path of the DAC protocol is the Nash equilibrium.
% \end{lemma}
% Proof is the same as the proof of Lemma~\ref{lem:security-one} since the payoffs of the DAC members do not depend on each other's actions.

% Although $\prm$ ensures that DAC security is satisfied in all Nash equilibria under certain assumptions, it could result in the slashing of DAC members even when the client receives a valid response to its query.
% Since DAC members could require occasional maintenance or be subjected to eclipse attacks, a desirable feature for the DAC protocol is to tolerate members that are temporarily offline as long as client queries are responded.
% Thus, a desired goal of the protocol in the presence of multiple DAC members is to ensure that non-responsive DAC members are slashed only when DAC security is violated.
% Towards this goal, consider a protocol $\prm$, where the contract slashes DAC members only if no valid response appears on the contract within $\Tcutoff$ rounds of a valid complaint being received.

% \begin{proposition}
% \label{prop:simple-optimal}
% Suppose $p_w<p_s$, there are $N$ DAC members, and there is a complaint on the contract.
% Consider an adversary that offers each DAC member $\node_i$, $i \in [N]$, $p^i_b$, and in return, asks them to avoid responding to a complaint on the contract.
% Then, given the constants $\alpha_i \in \mathbb{R}$, and the constraint
% \begin{equation*}
%     \sum_{i=1}^N \alpha_i p^i_b \leq p_0 < N(p_s-p_w),
% \end{equation*}
% the bribe allocation that maximizes the probability that there is no response on the contract in the Nash equilibrium is uniform:
% \begin{equation*}
%     p^i_b = \frac{p_0}{\sum_{i=1}^N \alpha_i}\ \forall i \in [N].
% \end{equation*}
% In this case, the maximum probability becomes
% \begin{equation*}
% \left(\frac{p_w+\frac{p_0}{\sum_{i=1}^N \alpha_i}}{p_s}\right)^{\frac{N}{N-1}}.
% \end{equation*}
% \end{proposition}

% \begin{proof}
% In the case a valid complaint appears on the contract at round $r'$, $\node_i$ can choose between sending a valid response to the contract by round $r'+\Tcutoff-\Tconf$, denoted by $\textsc{Respond-Contract}$, and withholding its response, denoted by $\textsc{Not-Respond}$.
% Let $q_{-i}$ denote the probability that excluding $\node_i$, no DAC member responds to the complaint on the contract in the equilibrium.
% Then, payoff of the actions $\textsc{Respond-Contract}$ and $\textsc{Not-Respond}$ are given by $-p_w$ and $p^i_b-p_s q^{-i}$.

% Suppose each DAC member $\node_j$, $j \in [N]$, $j \neq i$, independently chooses $\textsc{Respond-Contract}$ with probability $q_j$ and $\textsc{Not-Respond}$ with probability $1-q_j$.
% Then, the payoffs of the two actions become equal for $\node_i$ when $-p_w = p^i_b - p_s \prod_{j \in [N],j \neq i}(1-q_j)$.
% In this case, $\node_i$ can randomize over the two actions with any probability $q_i$ and $1-q_i$ in the equilibrium.
% Hence, in the equilibrium, for all $i \in [N]$, the probabilities $q_i$ satisfy $-p_w = p^i_b - p_s \prod_{j \in [N],j \neq i}(1-q_j)$, and
% \begin{equation*}
% \prod_{j \in [N],j \neq i}(1-q_j) = \frac{p^i_b + p_w}{p_s}.    
% \end{equation*}
% Multiplying these expressions, we obtain
% \begin{equation*}
% \left(\prod_{i \in [N]}(1-q_i)\right)^{N-1} = \prod_{i \in [N]} \frac{p^i_b + p_w}{p_s}.    
% \end{equation*}
% Hence, in the equilibrium, the probability that there is no response on the contract becomes
% \begin{equation*}
% \left(\prod_{i \in [N]} \frac{p^i_b + p_w}{p_s}\right)^{\frac{1}{N-1}}.    
% \end{equation*}

% Finally, given the constraint,
% \begin{equation*}
%     \sum_{i=1}^N \alpha_i p^i_b \leq p_0 < N(p_s-p_w),
% \end{equation*}
% the probability above is maximized if $p^i_b=p_0/(\sum_{i=1}^N \alpha_i)$ for all $i \in [N]$.
% Thus, the bribe allocation that maximizes the probability that there is no response on the contract in the Nash equilibrium is uniform:
% \begin{equation*}
%     p^i_b = \frac{p_0}{\sum_{i=1}^N \alpha_i}\ \forall i \in [N].
% \end{equation*}
% In this case, the maximum probability becomes
% \begin{equation*}
% \left(\frac{p_w+\frac{p_0}{\sum_{i=1}^N \alpha_i}}{p_s}\right)^{\frac{N}{N-1}}.
% \end{equation*}
% \end{proof}

% \begin{lemma}
% \label{lem:respond-optimal-1}
% Suppose
% \begin{equation*}
% \Tconf+\Texp+\Delta < \Tcutoff < \Tda,
% \end{equation*}
% \begin{equation*}
% p_1 < \min{(p_f,p_{\mathrm{comp}})-p_c},
% \end{equation*}
% \begin{equation*}
% p_0 < N(p_s - p_w).
% \end{equation*}
% Suppose the DAC consists of $N$ members and there is a single client. Then, the DAC security of Definition~\ref{def:dac-security} is satisfied except with probability
% \begin{equation*}
% q_{\mathrm{fail}} = \left(\frac{p_w+\frac{p_0}{N}}{p_s}\right)^{\frac{N}{N-1}}
% \end{equation*}
% in all Nash equilibria.
% \end{lemma}

% \begin{proof}
% Suppose the client $\client$ sends a valid query for the first time at round $r$.
% Towards contradiction, suppose there exists a Nash equilibrium, where DAC security (\cf Definition~\ref{def:dac-security}) is not satisfied with probability greater than $q_{\mathrm{fail}}$.

% Consider the case $\client$ does not hear a valid response over the network to its query by round $r+2\Delta$.
% In this case, suppose $\client$ does not send a valid complaint to the contract during the period $[r,r+\Tcutoff-\Tconf-\Texp-\Delta]$.
% Then, its maximum payoff becomes $p_1$.
% If $\client$ have sent the complaint to the smart contract by round $r+\Tcutoff-\Tconf-\Texp-\Delta$, it would have been received by the contract by round $r+\Tcutoff-\Texp-\Delta$.
% Then, by round $r+\Tcutoff-\Delta$, either the valid response would have been received by the contract, in which case $\client$ learns it by round
% $r+\Tcutoff$, or there would be no valid response sent to the contract, in which case $\client$ is credited $p_\mathsf{comp}$.
% In the first case, client obtains a payoff of $p_f-p_c$; in the latter, $p_\mathsf{comp}-p_c$.
% As $p_1 < \min{(p_f,p_\mathsf{comp})}-p_c$, this is a contradiction.
% Hence, in the Nash equilibrium, if $\client$ does not hear a valid response over the network to its query by round $r+2\Delta$, it sends a valid complaint to the contract during the period $[r,r+\Tcutoff-\Tconf-\Texp-\Delta]$.

% Towards contradiction, suppose there exists a Nash equilibrium such that a valid complaint is received by the contract at some round $r'$, and DAC security is violated with probability greater than $q_{\mathrm{fail}}$.
% Let $\mathcal{A}$ denote the PPT adversary of this Nash equilibrium.
% Suppose $\mathcal{A}$ offers each DAC member $\node_i$, $i \in [N]$, a bribe of $p^{\mathcal{A}}_i$ such that $\sum_{i \in [N]} p^{\mathcal{A}}_i < N(p_s-p_w)$, in return for following the strategy dictated by $\mathcal{A}$.
% Adversarial strategy for $\node_i$, $i \in [N]$, is parameterized by the probability $q^{\mathcal{A}}_i$ with which $\mathcal{A}$ dictates $\node_i$ to choose the action $\textsc{Respond-Contract}$\footnote{We assume that $\mathcal{A}$ can determine with certainty which DAC members follow the adversarial strategy, and rewards those DAC members at the end of the game.}.
% Let $q^{\mathcal{A}}$ denote the probability that no DAC member responds to the complaint on the contract in the equilibrium.
% Let $q^{\mathcal{A}}_{-i}$ denote the probability that excluding $\node_i$, no DAC member responds to the complaint on the contract in the equilibrium.
% Thus, $q^{\mathcal{A}}_{-i} \geq q^{\mathcal{A}}$ for all $i \in [N]$.

% Upon following the adversary's directives, each DAC member $\node_i$ receives a payoff of $p^{\mathcal{A}}_i$.
% If $\node_i$ takes the action $\textsc{Respond-Contract}$, it receives an additional payoff of $-p_w$, whereas if it takes the action $\textsc{Not-Respond}$, it receives an additional expected payoff of $-p_s q^{\mathcal{A}}_{-i}$.

% As DAC security is violated with probability exceeding $q_{\mathrm{fail}}$, then $q^{\mathcal{A}}>q_{\mathrm{fail}}>0$.
% Thus, no DAC member $\node_i$, $i \in [N]$, chooses $\textsc{Respond-Contract}$ with probability $1$ in the equilibrium.
% Now, suppose $-p_w \geq -p_s q^{\mathcal{A}}_{-i}$ in the equilibrium.
% Then, $q^{\mathcal{A}}_i < 1$ for all $i \in [N]$, and no DAC member chooses $\textsc{Not-Respond}$ with probability $1$ unless $q^{\mathcal{A}}_i=0$.
% Hence, it must be the case that $-p_w \leq p^{\mathcal{A}}_i+(-p_w q^\mathcal{A}_i-p_s q^{\mathcal{A}}_{-i} (1-q^{\mathcal{A}}_i))$ for all $i \in [N]$, which can be restated as
% \begin{equation*}
% -p_w \leq \frac{p^{\mathcal{A}}_i}{1-q^{\mathcal{A}}_i}-p_s q^{\mathcal{A}}_{-i}.
% \end{equation*}

% Consider an adversary $\mathcal{A}'$ such that $q^{\mathcal{A}'}_i = 0$ and $p^{\mathcal{A}'}_i = p^{\mathcal{A}'}_i/(1-q^{\mathcal{A}}_i)$.
% If a DAC member $\node_i$ chooses the actions $\textsc{Respond-Contract}$ and those dictated by $\mathcal{A}'$ with probabilities $q_i$ and $1-q_i$ in the equilibrium, then, it randomizes over the actions $\textsc{Respond-Contract}$ and those dictated by $\mathcal{A}$ with the same probabilities $q_i$ and $1-q_i$ in the equilibrium.
% Thus, $q^{\mathcal{A}} = q^{\mathcal{A'}}\prod_{i=1}^N(1-q^{\mathcal{A}}_i)$.

% We next consider the behavior of the DAC members given $\mathcal{A'}$.
% Given an allocation of bribes $p^{\mathcal{A'}}_i$, $i \in [N]$, suppose each $\node_i$, $i \in [N]$, randomizes over the actions $\textsc{Respond-Contract}$ and $\textsc{Not-Respond}$ with probabilities $q_i$ and $1-q_i$ respectively in the equilibrium.
% In this case, $q^{\mathcal{A'}} = \prod_{i \in [m]} (1-q_i)$ and $q^{\mathcal{A'}}_{-i} = \prod_{j \in [m]/\{i\}} (1-q_j)$.
% By Proposition~\ref{prop:simple-optimal}, given the constraint 
% \begin{equation*}
% \sum_{i=1}^N (1-q^{\mathcal{A}}_i)p^{\mathcal{A'}}_i = p_0 < N(p_s-p_w),
% \end{equation*} 
% the bribe allocation that maximizes $q^{\mathcal{A'}}$ is uniform:
% \begin{equation*}
% p^{\mathcal{A'}}_i = \frac{p_0}{N-\sum_{i=1}^N q^{\mathcal{A}}_i}
% \end{equation*}
% for all $i \in [N]$.
% By the same proposition, in this case, 
% \begin{equation*}
% q^{\mathcal{A'}} = \left(\frac{p_w+\frac{p_0}{(N-\sum_{i=1}^N q^{\mathcal{A}}_i)}}{p_s}\right)^{\frac{N}{N-1}},
% \end{equation*}
% which implies
% \begin{equation*}
% q^{\mathcal{A}} = q^{\mathcal{A'}} \prod_{i=1}^N(1-q^{\mathcal{A}}_i) = \left(\frac{p_w+\frac{p_0}{(N-\sum_{i=1}^N q^{\mathcal{A}}_i)}}{p_s}\right)^{\frac{N}{N-1}} \prod_{i=1}^N(1-q^{\mathcal{A}}_i),
% \end{equation*}
% The above expression is maximized when $q^{\mathcal{A}}_i = 0$ for all $i \in [N]$, which shows that $q^{\mathcal{A}} \leq q_{\mathrm{fail}} = ((p_w+\frac{p_0}{N})/p_s)^{N/(N-1)}$.
% Moreover, in the equilibrium where $q^{\mathcal{A}}$ is maximized, it is indeed true that $-p_w \geq -p_s q^{\mathcal{A}}_{-i}$.
% However, the statement $q^{\mathcal{A}} \leq q_{\mathrm{fail}}$ contradicts with the earlier assumption on $q^{\mathcal{A}}$.
% Consequently, there is no Nash equilibrium such that a valid complaint is received by the contract at some round $r'$, and DAC security is violated with probability greater than $q_{\mathrm{fail}}$.

% Finally, if DAC security is not satisfied in the Nash equilibrium with probability greater than $q_{\mathrm{fail}}$, $\client$ must not have heard a valid response over the network by round $r+2\Delta$, and must have sent a valid complaint to the contract during the period $[r,r+\Tcutoff-\Tconf-\Texp-\Delta]$ with probability at least $q_{\mathrm{fail}}$.
% In this case, a valid response for the complaint must have been sent to the contract by round $[r,r+\Tcutoff-\Delta]$ with probability greater than $q_{\mathrm{fail}}$.
% Thus, in any equilibrium, $\client$ learns about the valid response to its query by round $r+\Tcutoff<r+\Tda$ except with probability $q_{\mathrm{fail}}$.
% \end{proof}

% Note that at each query, a client $\client$ learns the valid response with probability at least $1-q_{\mathrm{fail}}$.
% Suppose $m(\Tconf+\Texp+3\Delta) < \Tcutoff$, and $\Tcutoff < \Tda$.
% Consider an honest client that repeatedly runs the DAC protocol with the same query if it does not receive a valid response within $\Tconf+\Texp+3\Delta$ rounds of its previous query.
% Then, by Lemma~\ref{lem:security-multiple}, DAC security is satisfied except with probability $q^m_{\mathrm{fail}}$.
% Hence, the latency period for DAC security can be adjusted as a function of the error rate $\epsilon$: 
% \begin{equation*}
% \Tda = \frac{\ln(\epsilon)}{\ln(q_{\mathrm{fail}})}(\Tconf+\Texp+3\Delta) = \frac{N-1}{N} \frac{\ln(\epsilon)}{\ln(p_w+\frac{p_0}{N})-\ln(p_s)}(\Tconf+\Texp+3\Delta).
% \end{equation*}

% \begin{lemma}
% \label{lem:respond-1}
% Suppose $p_w<p_s$ and there are $N$ DAC members.
% Consider an adversary that offers each DAC member $p_w$, and in return, asks them to avoid responding to a query over the network. 
% Moreover, assume that the client always complains through the contract when it does not receive a response over the network.
% Then, there exists a Nash equilibrium where DAC security is violated with probability $p_w/p_s$.
% \end{lemma}

% \begin{proof}
% Suppose that there exists a Nash equilibrium, where DAC members accept the adversary's bribe and do not respond to a client's query over the network.
% Thus, the client sends a complaint to the contract, through which the adversary understands that there has not been any response over the network.
% In this case, consider the strategy space of a DAC member $\node_i$, which can choose between two actions, $\textsc{Respond}$, \ie, responding on the contract, and $\textsc{Not-Respond}$.
% Let $q_n$ denote the probability that no DAC member other than $\node_i$ responds to the complaint.
% If $\node_i$ chooses $\textsc{Respond}$, its payoff becomes $0$.
% If it chooses $\textsc{Not-Respond}$, its payoff becomes $p_w-q_n p_s$.

% Suppose each DAC member other than $\node_i$ independently chooses $\textsc{Respond}$ with probability $q$ and $\textsc{Not-Respond}$ with probability $1-q$.
% Then, the payoffs of the two strategies become equal when $p_w-(1-q)^{N-1}p_s = 0$.
% Solving for the value of $q$ that satisfies the above equality gives
% \begin{equation*}
% q^* = 1-\left(\frac{p_w}{p_s}\right)^{\frac{1}{N-1}}.
% \end{equation*}
% Note that this strategy of randomizing over the two actions with probabilities $q^*$ and $1-q^*$ is a subgame perfect equilibrium.
% Moreover, in this equilibrium, expected payoff of each DAC member becomes 
% \begin{equation*}
% (1-q^*)(p_w-(1-q^*)^{N-1}p_s) = 0.
% \end{equation*}
% Consequently, no DAC member has an incentive to deviate to the strategy of responding over the network, in which case the payoffs are zero.
% Hence, there exists a Nash equilibrium, where no DAC member responds over the network and each DAC member responds on the contract independently with probability $q^*$.

% Finally, in this Nash equilibrium, with probability $(1-q^*)^N>0$, there would be no response to a query on the contract.
% Hence, there exists an equilibrium under which the client does not learn the correct response with probability
% \begin{equation*}
% (1-q^*)^N = \left(\frac{p_w}{p_s}\right)^{\frac{N}{N-1}},
% \end{equation*}
% and DAC security is violated.
% \end{proof}

% For a given $N$, the adversary following the starategy above has to give away
% \begin{equation*}
% p_0 = Np_w    
% \end{equation*}
% to violate DAC security with probability
% \begin{equation*}
% \left(\frac{p_w}{p_s}\right)^{\frac{N}{N-1}}.
% \end{equation*}
% Although the funds adversary needs to spend increases in $p_w$ and $N$, the failure probability also increases in $p_w$ and $N$.
% For instance, for $N=2$, $p_0 = 2p_w << p_s$, and $(p_w/p_s)^2$ is a non-negligible constant.
% Moreover, as the following lemma indicates, the adversary can adjust the probability of attack as a function of the bribes given to the DAC members.

% \begin{lemma}
% \label{lem:respond-2}
% Suppose $p_w<p_s$ and there are $N$ DAC members.
% Consider an adversary that offers each DAC member $p_b  \leq p_s-p_w$, and in return, asks them to avoid responding to a query over the network \emph{and} through the contract.
% Moreover, assume that the client always complains through the contract when it does not receive a response over the network.
% Then, there exists a Nash equilibrium where DAC security is violated with constant probability
% \begin{equation*}
% p_{\mathrm{fail}} = \left(\frac{p_b}{p_s}\right)^{\frac{N}{N-1}}
% \end{equation*}
% \end{lemma}

% \begin{proof}
% Suppose that there exists a Nash equilibrium, where some DAC members accept the adversary's bribe and do not respond to a client's query.
% Consider the strategy space of a DAC member $\node_i$.
% It can first choose between two actions, $\textsc{Respond-Network}$, \ie, responding over the network, and $\textsc{Not-Respond-Network}$. 
% In the case that no DAC member responds over the network, the client sends a complaint to the contract.
% In this case, $\node_i$ can choose between $\textsc{Respond-Contract}$, \ie, responding on the contract, and $\textsc{Not-Respond}$.

% Let $q^1_n$ denote the probability that no DAC member other than $\node_i$ responds to the query over the network.
% If no DAC member including $\node_i$ responds to the query over the network, the client sends a complaint to the contract.
% Conditioned on this event, let $q^2_n$ denote the probability that no DAC member other than $\node_i$ responds to the complaint over the network.

% Suppose each DAC member other than $\node_i$ independently chooses the action $\textsc{Respond-Network}$ with probability $q_r$, and if there is a complaint on the contract, independently chooses $\textsc{Respond-Contract}$ with probability $q_c$ and $\textsc{Not-Respond}$ with probability $1-q_c$.
% Conditioned on the event that there is a complaint on the contract, if $\node_i$ chooses $\textsc{Respond-Contract}$, its expected payoff becomes $-p_w$, and
% if it chooses $\textsc{Not-Respond}$, its expected payoff becomes $p_b-p_s q^2_n = p_b - p_s (1-q_c)^{n-1}$.
% These payoffs become equal when $-p_w = p_b-p_s(1-q_c)^{N-1}$.
% Solving for the value of $q_c$ that satisfies this equality, we obtain
% \begin{equation*}
% q_c^* = 1-\left(\frac{p_b + p_w}{p_s}\right)^{\frac{1}{N-1}}.
% \end{equation*}
% Thus, if $\node_i$ adopts the same strategy that randomizes over $\textsc{Respond-Contract}$ and $\textsc{Not-Respond}$, its expected payoff conditioned on the complaint event becomes $-p_w$.
% Conditioned on this event, the strategy of randomizing over $\textsc{Respond-Contract}$ and $\textsc{Not-Respond}$ with probability $q^*_c$ is a subgame perfect equilibrium.

% If $\node_i$ chooses $\textsc{Respond-Network}$, its payoff becomes $0$.
% On the other hand, if $\node_i$ chooses $\textsc{Not-Respond-Network}$ and no complaint appears on the contract, \ie, if another DAC member responds over the network, $\node_i$ gains a rewards of $p_b$ (Suppose the adversary can identify which DAC member responded over the network).
% Hence, if $\node_i$ chooses $\textsc{Not-Respond-Network}$, and adopts the above strategy for interacting with the contract, its expected payoff becomes
% \begin{equation*}
% (1-q^1_n)p_b + q^1_n (-p_w) = (1-(1-q_r)^{N-1})p_b + (1-q_r)^{N-1}(-p_w).
% \end{equation*}
% Thus, the payoffs of the actions $\textsc{Respond-Network}$ and  $\textsc{Not-Respond-Network}$ become equal when
% \begin{equation*}
% 0 = (1-(1-q_r)^{N-1})p_b + (1-q_r)^{N-1}(-p_w).
% \end{equation*}
% Solving for the value of $q_r$ that satisfies this equality, we obtain
% \begin{equation*}
% q_r^* = 1-\left(\frac{p_b}{p_b + p_w}\right)^{\frac{1}{N-1}}
% \end{equation*}
% Thus, if $\node_i$ also adopts the same strategy as the other DAC members that randomizes over $\textsc{Respond-Network}$ and $\textsc{Not-Respond-Network}$, its expected payoff becomes $0$.
% This strategy of randomizing over $\textsc{Respond-Network}$ and $\textsc{Not-Respond-Network}$ with probability $q^*_r$ is a Nash equilibrium.
% Hence, there exists a Nash equilibrium, where each DAC member could independently choose to not respond with probability $(1-q^*_r)(1-q^*_c)$.

% Finally, in this Nash equilibrium, with probability $(1-q^*_r)^N(1-q^*_c)^N>0$, there would be no response to the client's complaint.
% Hence, there exists a Nash equilibrium under which the client does not learn the correct response with probability
% \begin{equation*}
% p_{\mathrm{fail}} = (1-q^*_r)^N(1-q^*_c)^N = \left(\frac{p_b}{p_b + p_w}\right)^{\frac{N}{N-1}} \left(\frac{p_b + p_w}{p_s}\right)^{\frac{N}{N-1}} =  \left(\frac{p_b}{p_s}\right)^{\frac{N}{N-1}}
% \end{equation*}
% and DAC security is violated.
% \end{proof}

% For a given $N$, the adversary can violate DAC security with probability
% \begin{equation*}
% \left(\frac{p_b}{p_s}\right)^{\frac{N}{N-1}}
% \end{equation*}
% by spending in expectation
% \begin{equation*}
% N (1-q^*_r)(1-q^*_c)p_b = N \frac{(p_b+p_w)p_b}{p_s}.   
% \end{equation*}
% Although the funds adversary needs to spend in expectation increases in $p_b$ and $N$, the failure probability also increases in $p_b$ and $N$.

\subsection{Rewarding the Honest DAC Members}

To ensure that DAC security is satisfied with overwhelming probability, a reward scheme can be introduced.
We assume that the smart contract has a total initial supply of $T$, which it can distribute as reward to the DAC members responding to a client complaint on the contract.
Suppose that the contract distributes $T_n \leq T$ out of $T$ to the DAC members when there are $n$ responses on the contract within a $\Texp$ time window of the arrival of the query.
We assume that the DAC members run homogeneous processes for responding on the contract: If $n$ DAC members reply, then, in expectation, each DAC member receives $T_n/n$ reward.
For instance, if the contract chooses to reward the DAC member whose response appears first on the smart contract, then $T_n=T$ for all $n \in [N]$, and, when $n$ DAC members reply, each response attains the first position with probability $1/n$, implying an expected reward of $T_n/n$.
The homogeneity assumption enable us to simultaneously model different reward distribution schemes adopted by the contract.

Unfortunately, unless the rewards are high enough to offset the DAC's total cost $N p_w$ of responding on the smart contract, no reward scheme can ensure that the DAC security holds with overwhelming probability.
\begin{lemma}
\label{lem:respond-3}
Suppose there are $N$ DAC members.
Consider an adversary that offers each DAC member $p_w$, and in return, asks them to avoid responding to a query over the network.
Moreover, assume that the client always complains through the contract when it does not receive a response over the network.
Then, if $T < N p_w$, there exists a Nash equilibrium where DAC security is violated with constant probability $q_{\mathrm{fail}}$.
\end{lemma}

\begin{proof}
Suppose that there exists a Nash equilibrium, where DAC members accept the adversary's bribe and do not respond to a client's query over the network.
Thus, the client sends a complaint to the contract (through which the adversary understands that there has not been any response over the network).
In this case, consider the strategy space of a DAC member $\node_i$, which can choose between two actions, $\textsc{Respond}$, \ie, responding on the contract, and $\textsc{Not-Respond}$.
Let $q_k$ denote the probability that $k \in \{0,\ldots,N-1\}$, DAC members other than $\node_i$ responds to the complaint.
If $\node_i$ chooses $\textsc{Respond}$, its payoff becomes $\sum_{k=0}^{N-1} q_k \frac{T_{k+1}}{k+1}$.
If it chooses $\textsc{Not-Respond}$, its payoff becomes $p_w-q_0 p_s$.

Suppose each DAC member other than $\node_i$ independently chooses $\textsc{Respond}$ with probability $q$ and $\textsc{Not-Respond}$ with probability $1-q$.
Then, the payoff of the two actions become equal when 
\begin{equation*}
p_w - (1-q)^{N-1}p_s = \sum_{k=0}^{N-1} {N-1 \choose k} q^k (1-q)^{N-1-q} \frac{T_{k+1}}{k+1}. 
\end{equation*}
Let $\mathbf{q}(q)$, parametrized by the probability $q$, and $\mathbf{T}$ denote the vectors of length $N$, where the $i^{\text{th}}$ entry, $i \in \{0,\ldots,N-1\}$, is;
\[\begin{array}{rcl}
\mathbf{q}(q)[i] &=& {N-1 \choose i} q^i (1-q)^{N-1-i} \\
\mathbf{T}[i] &=& T_{i+1}/({i+1}) + p_s \mathbbm{1}_{i = 0}
\end{array}\]
Defining $\left<.,.\right>$ as the inner product of two vectors and using $\mathbf{q}$ and $\mathbf{T}$, we can express the equality above as follows:
\begin{equation}
\label{eq:prob}
p_w = \left< \mathbf{q}(q), \mathbf{T} \right>.
\end{equation}

If $T < N p_w$, there exists a number $q^* \in (0,1)$ that solves the equation~\ref{eq:prob}, and $q^*<1$. 
Then, the strategy of randomizing over the two actions with probability $q^*$ is a subgame perfect equilibrium.
Moreover, in this equilibrium, expected payoff of each DAC member becomes 
\begin{equation*}
p_w-(1-q^*)^{N-1}p_s > 0.
\end{equation*}
Consequently, no DAC member has an incentive to deviate to the strategy of responding over the network, in which case the expected payoff is zero.
Hence, there exists a Nash equilibrium, where no DAC member responds over the network and each DAC member responds on the contract independently with probability $q^*$.

Finally, in this Nash equilibrium, with probability $q_{\mathrm{fail}} = (1-q^*)^N>0$, there would be no response to a query on the contract.
Hence, there exists an equilibrium under which the client does not learn the correct response with constant positive probability, and DAC security is violated.
\end{proof}

Given the adversarial strategy above, the actual amount of bribe adversary has to pay to the DAC members depends on the probability $q_{\mathrm{fail}}$.
The proof shows that under this strategy,
\begin{equation*}
q_{\mathrm{fail}} = (1-q^*)^N,    
\end{equation*}
and the adversary has to pay at most
\begin{equation*}
p_w-(1-q^*)^{N-1}p_s = p_w - q_{\mathrm{fail}}^{\frac{N-1}{N}} p_s < p_w
\end{equation*}
to enforce the Nash equilibrium where the DAC security fails with probability $q_{\mathrm{fail}}$.

If $T \geq N p_w$, the reward scheme can ensure that the DAC members respond to complaints on the contract with probability $1$, in the absence of any bribe from the adversary.
In this case, if there is a complaint on the contract, each DAC member responds and is rewarded $T_{N-1}/N = T/N$ in expectation, with a total payoff of $T/N - p_w \geq 0$, which exceeds that of responding over the network.
However, such a reward scheme forces the contract to spend at least $N p_w$ funds per query appearing on the contract, some of which could have been sent by adversarial clients.
In particular, by compensating the cost $p_c$ of sending a complaint to the contract, adversary can ensure that a client sends a complaint even for queries that were answered over the network.
Hence, the adversary can drain $N p_w$ funds from the contract by only spending $p_c$ itself.
Similarly, rational DAC members would find it in their interest to withhold responses over the network, in order to gain rewards upon responding to a complaint on the contract.

\begin{lemma}
\label{lem:respond-4}
Suppose $p_w<p_s$ and there are $N$ DAC members.
Consider an adversary that offers each DAC member $p_b  \leq p_s-p_w$, and in return, asks them to avoid responding to a query over the network \emph{and} through the contract.
Moreover, assume that the client always complains through the contract when it does not receive a response over the network.
Then, if $T < N p_w$, there exists a Nash equilibrium where DAC security is violated with constant probability $q_{\mathrm{fail}}$.
\end{lemma}

\begin{proof}
Suppose that there exists a Nash equilibrium, where some DAC members accept the adversary's bribe and do not respond to a client's query.
Consider the strategy space of a DAC member $\node_i$.
It can first choose between two actions, $\textsc{Respond-Network}$, \ie, responding over the network, and \linebreak $\textsc{Not-Respond-Network}$. 
In the case that no DAC member responds over the network, the client sends a complaint to the contract.
In this case, $\node_i$ can choose between $\textsc{Respond-Contract}$, \ie, responding on the contract, and $\textsc{Not-Respond}$.

Let $q^1_n$ denote the probability that no DAC member other than $\node_i$ responds to the query over the network.
If no DAC member including $\node_i$ responds to the query over the network, the client sends a complaint to the contract.
Conditioned on this event, let $q^2_k$ denote the probability that $k \in \{0,\ldots,N-1\}$ DAC members other than $\node_i$ responds to the complaint on the contract.

Suppose each DAC member other than $\node_i$ independently chooses the action $\textsc{Respond-Network}$ with probability $q_r$, and if there is a complaint on the contract, independently chooses $\textsc{Respond-Contract}$ with probability $q_c$ and $\textsc{Not-Respond}$ with probability $1-q_c$.
Conditioned on the event that there is a complaint on the contract, if $\node_i$ chooses $\textsc{Respond-Contract}$, its expected payoff becomes
\begin{equation*}
-p_w + \sum_{k=0}^{N-1} {N-1 \choose k} q^k (1-q)^{N-1-q} \frac{T_{k+1}}{k+1},
\end{equation*}
and, if it chooses $\textsc{Not-Respond}$, its expected payoff becomes $p_b-p_s q^2_0 = p_b - p_s (1-q_c)^{n-1}$.
Then, the payoff of the two actions become equal when 
\begin{equation*}
p_w + p_b - (1-q)^{N-1}p_s = \sum_{k=0}^{N-1} {N-1 \choose k} q^k (1-q)^{N-1-q} \frac{T_{k+1}}{k+1}. 
\end{equation*}
Let $\mathbf{q}(q)$, parametrized by the probability $q$, and $\mathbf{T}$ denote the vectors of length $N$, where the $i^{\text{th}}$ entry, $i \in \{0,\ldots,N-1\}$, is;
\[\begin{array}{rcl}
\mathbf{q}(q)[i] &=& {N-1 \choose i} q^i (1-q)^{N-1-i} \\
\mathbf{T}[i] &=& T_{i+1}/({i+1}) + p_s \mathbbm{1}_{i = 0}
\end{array}\]
Defining $\left<.,.\right>$ as the inner product of two vectors and using $\mathbf{q}$ and $\mathbf{T}$, we can express the equality above as follows:
\begin{equation}
\label{eq:prob}
p_w+p_b = \left< \mathbf{q}(q), \mathbf{T} \right>.
\end{equation}

If $T < N (p_w+p_b)$, there exists a number $q^*_c \in (0,1)$ that solves the equation~\ref{eq:prob}, and $q^*_c<1$. 
Then, the strategy of randomizing over the two actions with probability $q^*_c$ is a subgame perfect equilibrium.
Moreover, in this equilibrium, expected payoff of each DAC member becomes
\begin{equation*}
p_b-(1-q^*_c)^{N-1}p_s.
\end{equation*}

If $\node_i$ chooses $\textsc{Respond-Network}$, its payoff becomes $0$.
On the other hand, if $\node_i$ chooses $\textsc{Not-Respond-Network}$ and no complaint appears on the contract, \ie, if another DAC member responds over the network, $\node_i$ gains a rewards of $p_b$ (Suppose the adversary can identify which DAC member responded over the network).
Hence, if $\node_i$ chooses $\textsc{Not-Respond-Network}$, and adopts the above strategy for interacting with the contract, its expected payoff becomes
\begin{equation*}
(1-q^1_n)p_b + q^1_n (p_b-(1-q^*_c)^{N-1}p_s) = (1-(1-q_r)^{N-1})p_b + (1-q_r)^{N-1}(p_b-(1-q^*_c)^{N-1}p_s).
\end{equation*}
Thus, the payoffs of the actions $\textsc{Respond-Network}$ and  $\textsc{Not-Respond-Network}$ become equal when
\begin{equation*}
0 = (1-(1-q_r)^{N-1})p_b + (1-q_r)^{N-1}(p_b-(1-q^*_c)^{N-1}p_s).
\end{equation*}
Solving for the value of $q_r$ that satisfies this equality, we obtain
\begin{equation*}
q_r^* = 1-\left(\frac{p_b}{p_b + (1-q^*_c)^{N-1}p_s}\right)^{\frac{1}{N-1}}
\end{equation*}
Thus, if $\node_i$ also adopts the same strategy as the other DAC members that randomizes over $\textsc{Respond-Network}$ and $\textsc{Not-Respond-Network}$, its expected payoff becomes $0$.
This strategy of randomizing over $\textsc{Respond-Network}$ and $\textsc{Not-Respond-Network}$ with probability $q^*_r$ is a Nash equilibrium.
Hence, there exists a Nash equilibrium, where each DAC member could independently choose to not respond with probability $(1-q^*_r)(1-q^*_c)$.

Finally, in this Nash equilibrium, with probability $(1-q^*_r)^N(1-q^*_c)^N>0$, there would be no response to the client's complaint.
Hence, there exists a Nash equilibrium under which the client does not learn the correct response with probability
\begin{equation*}
p_{\mathrm{fail}} = (1-q^*_r)^N(1-q^*_c)^N = \left(\frac{p_b(1-q^*_c)}{p_b + (1-q^*_c)^{N-1}p_s}\right)^{\frac{N}{N-1}}
\end{equation*}
and DAC security is violated.
\end{proof}

For a given $N$, the adversary can violate DAC security with probability
\begin{equation*}
p_{\mathrm{fail}} = \left(\frac{p_b(1-q^*_c)}{p_b + (1-q^*_c)^{N-1}p_s}\right)^{\frac{N}{N-1}}
\end{equation*}
by spending in expectation
\begin{equation*}
N \left(\frac{p^2_b(1-q^*_c)}{p_b + (1-q^*_c)^{N-1}p_s}\right).
\end{equation*}
Although the funds adversary needs to spend in expectation increases in $p_b$ and $N$, the failure probability also increases in $p_b$ and $N$.
Moreover, with this strategy, adversary drive up the total required reward to $N(p_b+p_w)$ as a linear function of its bribe.


% Let $c_1$ denote the total value stored by the accounts of the withdrawing clients.
% Let $c_2$ denote the total value staked by the DAC.
% Suppose $\client$s pay $c_3$ Eth to publish a complaint on chain.
% Similarly, suppose $\node$s pay $c'_3$ Eth to publish their proof on-chain.
% Let $c_4$ denote the financial cost (in terms of Eth) of calculating the SNARK proof for the circuit above.

% Suppose the DAC adopts a strategy where they never respond to queries for inclusion proofs, and upon observing a complaint on-chain, publish the SNARK proof with probability $1-x$.
% Thus, with probability $x$, DAC member ignore the complaint at the risk of slashing.
% Given this strategy, if honest clients decide to publish a complaint, they incur a cost $c_3$ with probability $1-x$ and $c_3+c_1$ with probability $x$.
% However, if $\client$s adopt a strategy of never publishing a complaint on-chain, they only incur a cost of $c_1$.
% Then, given the strategy above by $\node$s, complaining on-chain is dominated by inactivity as long as $c_1 < c_3(1-x)+(c_1+c_3)x$, i.e., $x>1-(c_3/c_1)$.
% Consequently, by choosing $x>1-(c_3/c_1)$, the DAC can ensure that the honest clients do not complain on-chain in the Nash equilibrium of this repeated game.
% In this case, honest clients incur a cost of $c_1$ whereas $\node$ do not incur any cost!
% Hence, for any level of bribe $c_0>0$, they will be willing to adopt this strategy.

% \subsection{Solution 1}
% To avoid the pathological situation above, honest clients can be forced to pay in advance for the cost of complaining on-chain.
% In this case, they will add the transaction fee $c_3$ of publishing a complaint on-chain to the dues paid to the DAC for its storage services.
% Then, if $\client$s complain on-chain; the trasaction fees for the complaint will be covered by the DAC from the dues payed by $\client$s.
% If there are no complaints on-chain, this sum is absorbed by $\node$s.

% As $\client$s incur the complaint cost $c_3$ regardless of the probability $x$, they will always find complaining to be the dominant strategy in the event that their queries are ignored.
% Hence, unless the bribe exceeds the stake, more generally, unless $c_0>c_2+c_3$, in the Nash equilibrium, the DAC will find it more profitable to reveal the inclusion proofs upon receiving a query.

% A major drawbacks of this solution is that clients always incur the cost $c_3$ of transaction fees.

% \ssubsection{Solution 2}
% To avoid the drawback above, an alternative and better solution is to ensure that clients are compensated for the cost $c_3$ of complaining on-chain when the DAC is slashed, potentially by receiving a portion $c_3+\delta$ of the slashed funds if $c_3+\delta<c_2$.
% In this case, if $c_1 \geq c_3$, complaining on-chain dominates inactivity for any probability $x$ defined above and chosen by the DAC as $c_1 = c_1(1-x) + c_1x \geq c_3(1-x) + (c_1-\delta)x = c_3(1-x)+(c_1+c_3-(c_3+\delta))x$ for any $x \in [0,1]$.
% Hence, again, unless the bribe exceeds the stake, more generally, unless $c_0>c_2+c_3$, in the Nash equilibrium, the DAC will find it more profitable to reveal the inclusion proofs upon receiving a query.

% \subsubsection{Drawbacks}
% \begin{itemize}
%     \item It requires the liveness of Ethereum for slashable safety, which weakens the premise of ZK rollups.
%     \item Malicious clients can force a rational DAC to pay $c'_3+c_4$ Eth by always complaining on-chain at the cost of $c_3$.
%     Thus, a briber can grief the DAC $c'_3+c_4$ amount of Eth by only paying $c_3$, which is potentially less than $c'_3+c_4$. 
%     Ideally, system should ensure that $c_3=c'_3+c_4$ to prevent such griefing opportunities against DAC members by malicious clients and against clients by malicious DAC members that are bribed.
% \end{itemize}


% At the beginning of the DAC protocol or any round thereafter, a client $\client$ can choose one or more of the following actions:
% \begin{itemize}
%     \item \textbf{Q1:} Send a valid query to the DAC through the network.
%     \item \textbf{Q2:} Send an invalid query to the DAC through the network.
%     \item \textbf{Q3:} Send a complaint with a valid query to the smart contract.
%     \item \textbf{Q4:} Send a complaint with an invalid query to the smart contract.
%     \item \textbf{R5:} Do not send anything to either the DAC or the smart contract.
% \end{itemize}
% At any round after the protocol commences, the DAC member $\node$ can choose one or more of the following actions:
% \begin{itemize}
%     \item \textbf{R1:} Send a valid response for a query through the network.
%     \item \textbf{R2:} Send an invalid response for a query through the network.
%     \item \textbf{R3:} Send a valid response for a query to the smart contract.
%     \item \textbf{R4:} Send an invalid response for a query to the smart contract
%     \item \textbf{R5:} Do not send anything to either the client or the smart contract.
% \end{itemize}
% The game is played for infinitely many rounds.
%
% For the sake of contradiction, suppose that there exists a Nash equilibrium, where DAC security (\cf Definition~\ref{def:dac-security}) is not satisfied.
% Thus, there exists a round $r$ such that $\client$ sent a valid query for the first time at round $r$, and has not learned the valid response by round $r+\Tda$.
% Since $\Tda > \Tcutoff$, in this case, $\client$'s total payoff can at most be $p_1$.
%
% Next, suppose that in the Nash equilibrium, $\client$ did not send a complaint with the valid query, \ie, a \emph{valid complaint} to the smart contract during the period $[r,r+\Tcutoff-\Tconf-\Texp-\Delta]$.
% If $\client$ had sent the complaint to the smart contract by round $r+\Tcutoff-\Tconf-\Texp-\Delta$, it would have been received by the contract by round $r+\Tcutoff-\Texp-\Delta$.
% Then, by round $r+\Tcutoff-\Delta$, either the valid response would have been received by the contract, in which case $\client$ learns it by round
% $r+\Tcutoff$, or there would be no valid response sent to the contract, in which case $\client$ is credited $p_\mathsf{comp}$ by the contract.
% In the first case, client would have obtained a payoff of $p_f-p_c$, in the latter $p_\mathsf{comp}-p_c$.
% As $p_1 < \min{(p_f,p_\mathsf{comp})}-p_c$, this is a contradiction.
% Hence, in the Nash equilibrium where DAC security is not satisfied, $\client$ must have sent a valid complaint to the contract during the period $[r,r+\Tcutoff-\Tconf-\Texp-\Delta]$.
%
% Finally, suppose a valid complaint is received by the contract at some round $r'$ in the Nash equilibrium, and $\node$ did not send a valid response to the contract by time $r'+\Tcutoff-\Tconf$.
% Then, the payoff of $\node$ can be at most $p_0-p_s$.
% However, if it had sent the valid response to the contract by time $r'+\Tcutoff-\Tconf$, its payoff would have been at least $-p_w$.
% Hence, as $p_0-p_s<-p_w$, in the Nash equilibrium where a valid complaint is received by the contract at some round $r'$, $\node$ must have sent a valid response by time $r'+\Tcutoff-\Tconf$.
%
% Finally, if DAC security is not satisfied in the Nash equilibrium, $\client$ must have sent a valid complaint to the contract during the period $[r,r+\Tcutoff-\Tconf-\Texp-\Delta]$, and $\node$ must have sent a valid response for the query to the contract by round $[r,r+\Tcutoff-\Delta]$.
% Thus, in the Nash equilibrium, $\client$ learns about the valid response to its query by round $r+\Tcutoff<r+\Tda$.
% However, this is a contradiction with the assumption that DAC security is not satisfied in the Nash equilibrium.
%
% \begin{center}
%     ***
%\end{center}
%
% For the second claim of the Lemma, observe that the payoffs of $\client$ and $\node$ are lower bounded by $p_f$ and $0$ respectively if they follow the DAC protocol.
% For the sake of contradiction, suppose $\node$ follows the DAC protocol, and $\client$ obtains a larger payoff by deviating from the protocol.
% Suppose $\client$ follows a strategy where it does not send a valid query to $\node$ for the first time over the network.
% This implies that $\client$ either does not send a valid query or complaint at all, or sends a valid complaint to the contract before it sends a valid query to $\node$ over the network.
% In the first case, $\client$'s payoff can at most be $p_1$ since $\node$ cannot send a valid response to an unknown query. 
% In the latter case, its payoff can at most be $p_1+\max{(p_f,p_{\mathrm{comp}})}-p_c$.
% Since both of these payoffs are smaller than $p_f$, $\client$ cannot increase its payoff by deviating from the DAC protocol.

% Next, suppose $\client$ follows the DAC protocol, and $\node$ receives a valid query from $\client$ over the network for the first time at some round $r'$.
% For the sake of contradiction, suppose $\node$ obtains a larger payoff by following a strategy where it does not send a valid response to $\client$ over the network at round $r'$.
% In this case, the payoff for the actions of $\client$ and the corresponding actions by $\node$ can be lower bounded as shown by the following table:
% \begin{center}
% \begin{tabular}{|c || c | c|} 
%  \hline
%   & Complain & Don't Complain \\ [0.5ex] 
%  \hline\hline
%  Response & $(p_f-p_c,-p_w)$ & - \\ 
%  \hline
%  No Response & $(p_{\mathrm{comp}}-p_c,-p_s)$ & $(0,0)$ \\ [1ex] 
%  \hline
% \end{tabular}
% \end{center}
% \vspace{1pt}
% Here, `complain' denotes the action where $\client$ sends a valid complaint to the contract, and `response' denotes the action where $\node$ sends the valid response to the contract.
% (There cannot be any response from $\node$ if no complaint is seen on the contract.)

% Consequently, as $\client$ follows the DAC protocol, it sends a valid complaint to the contract, in which case the payoff of $\node$ is upper bounded by $p_0-\max{(p_w,p_s)}$.
% Hence, as $p_0<\min{(p_w,p_s)}$, $\node$ cannot increase its payoff by deviating from the DAC protocol.

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
% Via table~\ref{tab:1}, we observe that regardless of the action profiles of all other nodes, none of the actions of the form, \eg, $P^i_1 \land P^i_2$, strictly dominates another action of the same form in terms of $\node_i$'s payoffs.
% Then, given the probabilities and events defined above, the payoff of a node $\node_i$, $i \in [N-f]$, can be expressed as follows:
% \begin{enumerate}
%     \item Under $P^i_1 \land P^i_2$: $(q_1+q_2)(-p_w)$.
%     \item Under $P^i_1 \land \overline{P}^i_2$: $(q_1+q_3)(-p_w)$. 
%     \item Under $\overline{P}^i_1 \land P^i_2$: $\leq (q_1+q_2)(-p_w-\epsilon)$.
%     \item Under $\overline{P}^i_1 \land \overline{P}^i_2$: $\leq (q_1+q_3)(-p_w-\epsilon)$.
% \end{enumerate}

% Via table~\ref{tab:2}, we observe that none of the actions of the form, \eg, $Q_1 \land Q_2$, strictly dominates another action of the same form in terms of the client's payoffs.
% Moreover, there exist action profiles for the nodes that are not strictly dominated by any other action profile within each event $P_1 \land P_2$, $\overline{P}_1 \land P_2$, $P_1 \land \overline{P}_2$, and $\overline{P}_1 \land \overline{P}_2$.
% Then, the client's expected payoff in the Nash equilibria can be expressed as follows:
% \begin{enumerate}
%     \item Under $Q_1 \land Q_2$: $(p_1+p_2+p_3)p_f - (p_1+p_2+p_3+p_4)p_c + (p_3+p_4) p_{\mathrm{comp}}$.
%     \item Under $\overline{Q}_1 \land Q_2$: $(p_1+p_3)p_f - (p_1+p_3)p_c + (p_3) p_{\mathrm{comp}}$. 
%     \item Under $Q_1 \land \overline{Q}_2$: $(p_1+p_2+p_3)p_f - (p_2+p_4)p_c + (p_4) p_{\mathrm{comp}}$.
%     \item Under $\overline{Q}_1 \land \overline{Q}_2$: $(p_1+p_3)p_f$.
% \end{enumerate}

% To find the probabilities $q_i$, $i \in [4]$, we set $\node_i$'s payoffs above to be equal and solve for $q_i$.
% This gives $q_1=q_2=q_3=0$ and $q_4=1$.
% On the other hand, to find the probabilities $p_i$, $i \in [4]$, we set the client's payoffs to be equal and solve for $p_i$ given the constraint $\sum_{i=1}^4 p_i = 1$.
% However, the equations 2 and 4 above together imply that $p_1 = \frac{p_{\mathrm{comp}-p_c}}{p_c} p_3$, and 1 and 4 together imply that $p_1 \geq \frac{p_{\mathrm{comp}}-p_c}{p_{\mathrm{comp}}}$.
% This gives $p_3 \geq \frac{p_c}{p_{\mathrm{comp}}}$, and $p_1 + p_3 \geq \frac{p_{\mathrm{comp}}}{p_c}\frac{p_c}{p_{\mathrm{comp}}} \geq 1$.
% Hence, $p_1+p_3=1$, $p_2+p_4=0$, and in the Nash equilibrium, the event $P_1$ happens with probability $1$.

%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%

% Suppose a query is received by the contract at the end of some slot $j \in \mathbb{N}$.
% Then, every node obtains a larger payoff by taking the action $\place$ rather than $\neg\place$ at slot $j+1$.
% Hence, there are more than $k$ valid clues in the contract at slot $j+1$ with probability $1$ in any Nash equilibria of the subgame where a query is received by the contract at slot $j$.

% Suppose $\client$ receives less than $k$ valid clues over the network by the end of slot $3$.
% Then, if $\client$ does not take the action $\query$ by slot $2$, $\client$'s payoff becomes at most $0$.
% Conversely, if $\client$ takes the action $\query$ by slot $2$, it obtains a payoff of at least $p_\mathrm{comp}-p_c$ when the game is terminated.
% (For risk-averse nodes, the minimum payoff is expressed as $(C+p_\mathrm{comp}-p_c)^\nu$.)
% Hence, if the action profile of the nodes cause less than $k$ valid clues to be sent to $\client$ over the network by slot $3$, as $p_\mathrm{comp}-p_c>0$ ($(C+p_\mathrm{comp}-p_c)^\nu>0$), $\client$ chooses to take the action $\query$ by slot $2$, and its payoff becomes at least $p_\mathrm{comp}-p_c$ ($(C+p_\mathrm{comp}-p_c)^\nu$ for risk-averse nodes).
% In this case, $\client$'s query is received by the contract at slot $2$.

% Finally, given any action profile where the nodes send at least $k$ valid clues to $\client$ over the network by slot $3$, $4$-security is satisfied.
% Conversely, given action profiles where they do not send sufficiently many valid clues by slot $3$, $\client$ takes the action $\query$ by slot $2$.
% However, if $\client$ takes the action $\query$ by slot $2$, nodes send $k$ or more valid clues to the contract by slot $3$.
% Consequently, we observe that in all action profiles that have not yet been strictly dominated, $4$-security is satisfied with probability $1$, implying that $4$-security is satisfied with probability $1$ in any Nash equilibria of the game.


%%%%%%%%%%%%%%%%%%%%%%%%
%Analysis that was made to find an upper bound on the error probability of our contract in the presence of risk-averse nodes
%%%%%%%%%%%%%%%%%%%%%%%%
% Without loss of generality, suppose $q_i \geq q_{i+1}$ for all $i \in [N-f-1]$.

% Any set $C \in \mathcal{C}$ that contains a node $\node_i$, $i \in [N-f-k]$, also contains a node $\node_j$, $j \in \{N-f-k+1,\ldots,N-f\}$.
% Then,
% \begin{IEEEeqnarray*}{C}
% \bigcup_{i=1}^{N-f}\bigcup_{C \in D_i} E_C \subseteq \bigcup_{i=N-f-k+1}^{N-f}\bigcup_{C \in D_i} E_C
% \end{IEEEeqnarray*}

% Using the observations above and the union bound, we can write 
% \begin{IEEEeqnarray*}{rCl} 
% q^{\mathcal{A}}_{\mathrm{v}} &=& \Pr\left[\bigcup_{C \in D_i} E_C\right] \\
% &=& \Pr\left[\bigcup_{i=1}^{N-f}\bigcup_{C \in D_i} E_C\right] \\
% &=& \Pr\left[\bigcup_{i=N-f-k+1}^{N-f}\bigcup_{C \in D_i} E_C\right] \\
% &\leq& \sum_{i=N-f-k+1}^{N-f} \Pr\left[\bigcup_{C \in D_i} E_C\right] \\
% &=& \sum_{i=N-f-k+1}^{N-f} q_i
% \end{IEEEeqnarray*}

% As $|C|=N-f-k+1$ for all $C \in \mathcal{C}$, for any $C \subseteq D_i$ and $i \in [N-f]$, there exist $N-f-k$ other nodes $\node_j$, $j \neq i$, $j \in [N-f]$, such that $C \in D_j$.
% Then, by union bound, we can also write
% \begin{IEEEeqnarray*}{rCl} 
% q^{\mathcal{A}}_{\mathrm{v}} &=& \Pr\left[\bigcup_{i=1}^{N-f}\bigcup_{C \in D_i} E_C\right] \\
% &\leq& \frac{1}{N-f-k+1} \sum_{i=1}^{N-f} \Pr\left[\bigcup_{C \in D_i} E_C\right] \\
% &=& \frac{1}{N-f-k+1} \sum_{i=1}^{N-f} q_i
% \end{IEEEeqnarray*}

% Combining the two inequalities, we obtain
% \begin{IEEEeqnarray*}{C} 
% q^{\mathcal{A}}_{\mathrm{v}} \leq \min\left(\frac{1}{N-f-k+1} \sum_{i=1}^{N-f} q_i,\ \sum_{i=N-f-k+1}^{N-f} q_i\right),
% \end{IEEEeqnarray*}
% where we can express $q_i$ as the function $f(p^i_b)$.
% Here,
% \begin{IEEEeqnarray*}{C}
% f(x) = \frac{(x + C-p_w)^\nu-(C-p_w)^\nu}{(x + C-p_w)^\nu-(x + C-p_s)^\nu}
% \end{IEEEeqnarray*}
% is non-negative, convex and increasing for all $\nu \in (0,1)$, and its domain is $[0,p_0]$.
% Then, for all $\epsilon > 0$, for any non-negative $x_1,x_2 \in [\epsilon,p_0-\epsilon]$ such that $x_1 > x_2$, it holds that $f(x_1)+f(x_2) \leq f(x_1 + \epsilon) + f(x_2-\epsilon)$.

% For any two sequences $p^i_b$, $i=1,\ldots,N-f$ and $p^i_{b'}$, $i=1,\ldots,N-f$ in $\mathbb{R}^{N-f}_+$ such that (i) $\sum_{i \in [N-f]} p^i_b = \sum_{i \in [N-f]} p^i_{b'} = p_0$, (ii) $p^i_{b'} \leq p^i_b$ for $i \in \{N-f-k+1,\ldots,N-f\}$, and (iii) $p^i_{b'} \geq p^i_{b}$ for all $i \in [N-f-k]$, it holds that
% \begin{IEEEeqnarray*}{C} 
% \sum_{i=1}^{N-f} f(p^i_{b'}) \leq \sum_{i=1}^{N-f} f(p^i_b).
% \end{IEEEeqnarray*}
% and, 
% \begin{IEEEeqnarray*}{C} 
% \sum_{i=N-f-k+1}^{N-f} f(p^i_{b'}) \geq \sum_{i=1}^{N-f} f(p^i_b).
% \end{IEEEeqnarray*}

% %Intersect the two inequalities, then find the optimal result.

% The bound above implies the existence of at least one node $\node_{i^*}$ such that $\mathbb{E}[U^*_{i^*}] < -p_w$.
% However, taking the action $\place$ at slot $j+1$ would give a payoff of $-p_w$ for $\node_{i^*}$ regardless of the actions of all other nodes, implying that there exists an action that strictly dominates the one taken by $\node_{i^*}$ in the equilibrium.
% Thus, we have reached a contradiction.
%%%%%%%%%%%%%%%%%%%%%%%%
